Sample-Optimal Average-Case Sparse Fourier Transform in Two Dimensions

We present the first sample-optimal sublinear time algorithms for the sparse Discrete Fourier Transform over a two-dimensional sqrt{n} x sqrt{n} grid. Our algorithms are analyzed for /average case/ signals. For signals whose spectrum is exactly sparse, our algorithms use O(k) samples and run in O(k log k) time, where k is the expected sparsity of the signal. For signals whose spectrum is approximately sparse, our algorithm uses O(k log n) samples and runs in O(k log^2 n) time; the latter algorithm works for k=Theta(sqrt{n}). The number of samples used by our algorithms matches the known lower bounds for the respective signal models. By a known reduction, our algorithms give similar results for the one-dimensional sparse Discrete Fourier Transform when n is a power of a small composite number (e.g., n = 6^t).

==> alg_1d.tex <==
\section{Exact 1D Algorithm for any sparsity $k$}
\label{sec:1d}
 
\begin{algorithm}[!htbp]
\caption{Exact 1D sparse FFT algorithm} \label{a:1d}
    \begin{algorithmic}
    \Procedure{Noiseless1DSparseFFT}{x,k}
        \State $B = \alpha k/\log{k}$, for some constant $\alpha$.
        \State $T \gets \{0, 1, \cdots, 2C\log{k}\}$, for some large constant $C$. 
        \For{$\tau \in T$}
            \State Compute the FFT $\wh{u}^{(\tau)}$ of $u^{(\tau)}$ where for $i \in [B]$, where $u^{(\tau)}_{i} = x_{i(n/B)+\tau} $
        \EndFor
        \State $\wh{z} \gets 0$
        \State Compute $J = \{j : |\wh{u}^{(\tau)}_j| > 1/2 \}$
        \For{$j \in J$}
            \State  $\Lambda(f) \gets \textsc{BerlekampMassey}(\wh{u}^{(T)}_j)$.
            \State  $\{f_0,f_1,\cdots,f_{C\log{k}}\} \gets \textsc{Pan}(\Lambda(f))$. \Comment{This finds $\{f : |\wh{x}_f| > 0\ \mbox{and}\ f = j \mod B\}$ } 
            \State  $V \gets \textsc{Vandermonde}(\omega^{f_1},\omega^{f_2},\cdots,\omega^{f_{C\log{k}}})$ \Comment{$\omega$ is $nth$ root of unity}
            \State  $V^{-1} \gets$ \textsc{InverseVandermonde}($V$) \Comment{Invert Vandermonde matrix}
            \State  $\{v_0,v_1,\cdots,v_{C\log{k}}\} \gets V^{-1}\wh{u}^{(T)}_j$
            \State  $\wh{z}_i \gets v_i$ for $i \in [C\log{k}]$.
        \EndFor
        \State \Return $\wh{z}$
    \EndProcedure
    \end{algorithmic}

\end{algorithm}

The algorithm \textsc{Noiseless1DSparseFFT}(Alg~\ref{a:1d}) works for 1D spectrum with any sparsity $k=O(n)$ with $O(k)$ samples
in $O(k\log{k})$ running time. The outline is as follows: 
We fold the spectrum into $k/\log{k}$ bins using the 1D version of the comb filter (section \xref{sec:defs}). 
For each of the bin, with high probability there are $O(\log{k})$ nonzero frequencies (Thereom~\ref{thm:1d_prob}). 
Our algorithm recovers these frequencies and their values in $O(\log^2{k})$ time, by the following combination of procedures:
\begin{itemize}
    \item \textsc{BerlekampMassey}: This procedure calculates the coefficients of the locator polynomial $\Lambda(f)$, 
        based on the value of the buckets. The locator polynomial, which determines the positions of the nonzero frequencies, 
        is defined as follows:
        \begin{equation}
            \label{equ:locator_poly}
            \Lambda(f) = \prod_{\ell=0}^{C\log{k}}\left(1-{z}\omega^{f_\ell}\right)
        \end{equation}
 % Removed    = \sum_{d=0}^{C\log{k}} c_dz^d , not needed
        Our algorithm employs the Berlekamp-Massey algorithm~\cite{massey1, massey2}: first, as shown in~\cite{reed-solomon}, 
        finding the positions of the nonzero frequencies is equivalent to a generalization of Reed-Solomon decoding problem in 
        complex field; then, solving this complex-field Reed-Solomon problem boils down to recovering lowest-order linear 
        recurrence ($\Lambda(f)$) generating a given sequence of ``syndromes''(the bins in our context)~\cite{coding-theory, 
        massey1}. Berlekamp-Massey solves this problem in quadratic time with regard to the order of $\Lambda(f)$, i.e., $O(\log^2{k})$.
    \item \textsc{Pan}: From the definition of locator polynomial (equation~\ref{equ:locator_poly}), the root of $\Lambda(f)$ 
        determines nonzero frequencies $\{f_0, f_1, \cdots, f_{C\log{k}}\}$. We adopt the Pan algorithm~\cite{pan87} to find
        the complex roots, which runs in time $O(d\log{d}\log{b})$, where $n$ is the order of the polynomial and $b$ is the
        precision. This results in a $O(\log{k}\log\log{k})$ algorithm. 
    \item \textsc{Vandermonde}: Given the nonzero frequencies, it's a linear system with regard to the values of these
        frequencies, and the coefficient matrix is Vandermonde. 
        \begin{equation}
            \label{equ:vandermonde}
            V \left[\begin{array}{c}v_0\\v_1\\\vdots\\v_{C\log{k}}\end{array}\right] = \wh{u}_j^{(T)}, 
            \mbox{\ where\ } V = \left[
            \begin{array}{cccc}
            1 & 1 & \cdots & 1\\
            \omega^{f_1} & \omega^{f_2} & \cdots & \omega^{f_{C\log{k}}}\\
            \omega^{2f_1} & \omega^{2f_2} & \cdots & \omega^{2f_{C\log{k}}}\\
            \vdots & \vdots & \ddots & \vdots\\
            \omega^{C\log{k}f_1} & \omega^{C\log{k}f_2} & \cdots & \omega^{C\log{k}f_{C\log{k}}}\\
            \end{array}\right]
        \end{equation}
    \item \textsc{InverseVandermonde}: Inverting Vandermonde can be done in time $O(d^2)$ if $d$ is the matrix is size $d\times{d}$~\cite{vandermonde}.
        This means we can find the values by inverting the Vandermonde matrix in time $O(\log^2{k})$ time. 
\end{itemize}

We have $k/\log{k}$ bins, each takes $O(\log{k})$ time to estimate the nonzero frequencies and their values, 
the running time is thus $O(k/\log{k}\cdot\log^2{k})=O(k\log{k})$. 
For each of the bins, we need $O(\log{k})$ shifts, so the total number of samples needed is 
$O(k/\log{k}\cdot\log{k})=O(k)$.

The correctness of the algorithm in average case is guaranteed by the following theorem: 

\begin{theorem}
\label{thm:1d_prob}
Under the Bernoulli assumptions and comb filter in seciton \xref{sec:defs}, 
for 1D-DFT with size $n$, we fold the spectrum into $B=k/\log{k}$ bins.
For large enough $C$, the probability that there is at most $C\log{k}$ supports 
hashing into any bin is smaller than $O((1/k)^{C\log{C}})$.
\end{theorem}

\begin{proof}
The probability that there is no bin with more than $m$ supports hashed into it 
when there is $B$ buckets and $k$ supports is bounded by~\cite{collision_prob}:
\textred{Badih: what is this citation?}
\begin{equation}
\label{equ:collision_prob}
\mbox{Pr}(B, k, m) \le B\left( \frac{ek}{Bm} \right)^m
\end{equation}
When $B=k/\log{k}$, $m=C\log{k}$, this boils down to 
$$\mbox{Pr}(B, k, m) \le B\left( \frac{ek}{Bm} \right)^m
\le \frac{k}{\log{k}}\left( \frac{e}{C} \right)^{C\log{k}}
= O\left(\frac1{k^{C\log{C}}}\right)$$
\end{proof}


==> alg_1d_2.tex <==
\section{Exact 1D Algorithm for any sparsity $k$}
\label{sec:1d}

\begin{algorithm}[!htbp]
\caption{Exact 1D sparse FFT algorithm} \label{a:1d}
    \begin{algorithmic}
    \Procedure{Noiseless1DSparseFFT}{x,k}
        \State $B = \alpha k/\log{k}$, for some constant $\alpha$.
        \State $T \gets \{0, 1, \cdots, 2C\log{k}\}$, for some large constant $C$. 
        \For{$\tau \in T$}
            \State Compute  the FFT $\wh{u}^{(\tau)}$ of $u^{(\tau)}$ where for every $i \in [B]$, $u^{(\tau)}_{i} = x_{i(n/B)+\tau} $
        \EndFor
        \State $\wh{z} \gets 0$
 %       \State Compute $J = \{j : |\wh{u}^{(\tau)}_j| > 1/2 \}$
        \For{$j \in [B]$} \xxx{Replaced $J$ by $[B]$, since all buckets will likely contain something}
            \State  $\Lambda(f) \gets \textsc{BerlekampMassey}(\wh{u}^{(T)}_j)$.
            \State  $\{f_0,f_1,\cdots,f_{C\log{k}}\} \gets \textsc{Pan}(\Lambda(f))$. \Comment{This finds $\{f : |\wh{x}_f| > 0\ \mbox{and}\ f = j \mod B\}$ } 
            \State  $V \gets \textsc{Vandermonde}(\omega^{f_1},\omega^{f_2},\cdots,\omega^{f_{C\log{k}}})$ %\Comment{$\omega$ is an $n$th root of unity}
            \State  $V^{-1} \gets$ \textsc{InverseVandermonde}($V$) \Comment{Invert Vandermonde matrix}
            \State  $\{v_0,v_1,\cdots,v_{C\log{k}}\} \gets V^{-1}\wh{u}^{(T)}_j$
            \State  $\wh{z}_{f_{i}} \gets v_i$ for all $i \in [C\log{k}]$.
        \EndFor
        \State \Return $\wh{z}$
    \EndProcedure
    \end{algorithmic}

\end{algorithm}

The algorithm \textsc{Noiseless1DSparseFFT}(Alg~\ref{a:1d}) works for 1D spectrum with any sparsity $k=O(n)$ with $O(k)$ samples
in $O(k\log{k})$ running time. The outline is as follows: 
We fold the spectrum into $k/\log{k}$ bins using the 1D version of the comb filter (section \xref{sec:defs}). 
With high probability, each of the bins has $O(\log{k})$ nonzero frequencies (Lemma~\ref{lem:1d_prob}). 
Our algorithm recovers these frequencies and their values in each bin by the following procedures:
\begin{itemize}
    \item \textsc{BerlekampMassey}: This procedure calculates the coefficients of the locator polynomial $\Lambda(f)$, 
        based on the values of the buckets. The locator polynomial, which is determined by the positions of the nonzero frequencies, 
        is defined as follows:
        \begin{equation}
            \label{equ:locator_poly}
            \Lambda(f) = \prod_{\ell=0}^{C\log{k}}\left(1-{z}\omega^{f_\ell}\right)
        \end{equation}
        
% removed  \sum_{t=0}^{C\log{k}} c_tz^t =  
        Recovering this locator polynomial resembles Reed-Solomon code~\cite{reed-solomon} except that it is 
        in the complex field. According to lemma~\ref{lem:massey}, Berlekamp-Massey algorithm~\cite{massey1} 
        solves this problem in quadratic time. 
    \item \textsc{Pan}: From the definition of the locator polynomial (equation~\ref{equ:locator_poly}), the roots of $\Lambda(f)$ 
        determine the nonzero frequencies $\{f_0, f_1, \cdots, f_{C\log{k}}\}$. We use the Pan algorithm~\cite{pan95} to find
        the complex roots, whose correctness and efficiency is guaranteed by lemma~\ref{lem:pan}.
    \item \textsc{Vandermonde}: Given the nonzero frequencies, the problem reduces to solving a linear system in the values of these
        frequencies. The coefficient matrix of this system is Vandermonde. 
        \begin{equation}
            \label{equ:vandermonde}
            V \left[\begin{array}{c}v_0\\v_1\\\vdots\\v_{C\log{k}}\end{array}\right] = \wh{u}_j^{(T)}, 
            \mbox{\ where\ } V = \left[
            \begin{array}{cccc}
            1 & 1 & \cdots & 1\\
            \omega^{f_1} & \omega^{f_2} & \cdots & \omega^{f_{C\log{k}}}\\
            \omega^{2f_1} & \omega^{2f_2} & \cdots & \omega^{2f_{C\log{k}}}\\
            \vdots & \vdots & \ddots & \vdots\\
            \omega^{C\log{k}f_1} & \omega^{C\log{k}f_2} & \cdots & \omega^{C\log{k}f_{C\log{k}}}\\
            \end{array}\right]
        \end{equation}
    \item \textsc{InverseVandermonde}: We use algorithm ~\cite{vandermonde}  to invert the linear system in order to estimate the values of the
    frequencies (Lemma~\ref{lem:invert_vandermonde}).
\end{itemize}

\noindent\textbf{Analysis of \textsc{Noiseless1DSparseFFT}}
The correctness of the algorithm in the average case is guaranteed by Theorem~\ref{thm:noiseless_1d_sparse_fft}.

\begin{lemma}
\label{lem:massey}
For a specific bin, if there are $t$ nonzero frequencies hashing to it, algorithm \textsc{BerlekampMassey} finds
the locator polynomial $\Lambda(f)$ (equation \ref{equ:locator_poly}) in time $O(t^2)$.
\end{lemma}
\begin{proof}
First, as shown in~\cite{reed-solomon}, 
finding the positions of the nonzero frequencies is equivalent to a generalization of the Reed-Solomon decoding problem to 
complex fields; then, solving this complex-field Reed-Solomon problem reduces to recovering lowest-order linear 
recurrence ($\Lambda(f)$) that generates a given sequence of ``syndromes'' (the bins in our context)~\cite{coding-theory}.
The running time is quadratic to the order of the polynomial, i.e., $O(t^2)$~\cite{massey1}.
\end{proof}

\begin{lemma}
\label{lem:pan}
For a polynomial with complex coefficients and order $t$, and whose complex roots are confined within the unit disk 
$\{x : |x| \le 1\}$, \textsc{Pan} approximate all of the roots (absolute error bound $2^{-b}$) with order of $n$ 
arithmetic operations $O(t\log^2{t}(\log^2{t}+\log{b})$.
\end{lemma}
\begin{proof}
This is shown in paper~\cite{pan95}.
\end{proof}

\begin{lemma}
\label{lem:invert_vandermonde}
Given a $t\times{t}$ Vandermonde matrix $V$, its inverse can be calculated in time $O(t^2)$.
\end{lemma}
\begin{proof}
This is shown in paper~\cite{vandermonde}.
\end{proof}

\begin{lemma}
\label{lem:1d_prob}
Under the Bernoulli assumptions of $k$-sparsity of $\wh{x}$ in section \xref{sec:defs}.
If we fold the spectrum into $B=k/\log{k}$ bins, then for large enough $C$, the probability that there is a bin with more than $C\log{k}$ nonzero frequency components hashing to it is smaller than $O((1/k)^{0.5C\log{C}})$.
\end{lemma}
\begin{proof}
The probability $\mbox{Pr}(B, k, m)$ that there is a bin with at least $m$ nonzero frequency components hashing to it is bounded by:
%\textred{Do we need a citation here?}
\begin{equation}
\label{equ:collision_prob}
\mbox{Pr}(B, k, m) \le B {n/B \choose m} \left(\frac{k}{n}\right)^{m} \le B \left( \frac{ek}{Bm} \right)^m 
\end{equation}
Since $B=k/\log{k}$, $m=C\log{k}$, we get: 
$$\mbox{Pr}(B, k, m) \le B\left( \frac{ek}{Bm} \right)^m
\le \frac{k}{\log{k}}\left( \frac{e}{C} \right)^{C\log{k}}
= O\left(\frac1{k^{0.5C\log{C}}}\right)$$
\end{proof}

\begin{theorem}
\label{thm:noiseless_1d_sparse_fft}
Under the Bernoulli assumptions of $k$-sparsity of $\wh{x}$ in section \xref{sec:defs}, 
the algorithm \textsc{Noiseless1DSparseFFT} runs in $O(k(\log{k}+\log^2\log{k}\log\log{n})$
time with $O(k)$ samples, and returns the correct spectrum $\wh{x}$ with probability 
at least $O(1/k^2)$.
\end{theorem}
\begin{proof}
From lemma~\ref{lem:1d_prob}, we pick $C$ large enough, such that the probability 
that there is a bin with more than $C\log{k}$ is below $O(1/k^2)$. Now we need
to show that with at most $C\log{k}$ supports in each bin, we can recover them 
in time $O(k\log{k})$ with $O(k)$ samples. 

From lemma~\ref{lem:massey},~\ref{lem:invert_vandermonde}, the running time
is $O(t^2)$ for each bin with at most $t$ nonzero frequencies, to finish
the \textsc{BerlekampMassey}, \textsc{Vandermonde} and \textsc{InverseVandermonde}
subprocedure. For the root finding algorithm \textsc{Pan}, the running time
is $O(t\log^2{t}(\log^2{t}+\log{b})$ with precision $2^{-b}$. Since the roots are 
$\sqrt{n}$-th root of unity, $O(1/\sqrt{n})$ precision suffices. 
For our case, $t=C\log{k}$, the running time for each bin will be $O(\log^2{k})$.
Therefore, the total running time is $O(B(\log^2{k}+\log{k}\log^2\log{k}\log\log{n})=O(k(\log{k}+\log^2\log{k}\log\log{n}))$.

For each of the bins, we need $O(\log{k})$ shifts ($|T|=O(\log{k})$), so the total number 
of samples needed is $O(k/\log{k}\cdot\log{k})=O(k)$.
\end{proof}





==> alg_inf_SNR_general_k.tex <==
\subsection{Exact Algorithm: $k = O(\sqrt{n})$}

\xxx{This section might get replaced by a reduction to  the case $k=\Theta(\sqrt{n})$}
The algorithm \textsc{Noiseless2DSparseFFT} is described as Algorithm~\ref{a:exact}.
This algorithm is very similar to the basic algorithm. The difference is that it needs
to fold the spectrum into $k \le c\sqrt{n}$ bins for some constant $c$. 
Instead of folding into a row or column of size $\sqrt{n}$, it further folds the row
or column by $\sqrt{n}/k$ into $k$ bins. As a result, it requires two time shifts
- one vertical and another horizontal- to estimate the row and column indices of a 
large frequency that was folded into a bin.  


\begin{algorithm}[t!]
 \caption{Exact 2D sparse FFT algorithm for $k = O(\sqrt{n})$}\label{a:exact}
  \begin{algorithmic}
    \Procedure{EstimateFreq}{$\wh{u}^{(T)}$, $\wh{v}^{(T)}$, $T$, $B$, IsCol}
    \State $\wh{w} \gets 0$.
    \State Compute $J=\{j: |\wh{u}^{(0)}_j| > 1/2\}$.
    \For{$j \in J$}
    \State $b \gets \wh{u}^{(0,0)}_{j} / \wh{u}^{(1,0)}_{j}$.
    \State $b' \gets \wh{u}^{(0,0)}_{j} / \wh{u}^{(0,1)}_{j}$.
    \State $i  \gets \text{round}(\phi(b)\frac{\sqrt{n}}{2\pi}) \bmod \sqrt{n}$.
    \State $i'  \gets \text{round}(\phi(b')\frac{\sqrt{n}}{2\pi}) \bmod \sqrt{n}$.

    \State $a \gets \text{round}(\wh{u}^{(0,0)}_{j})$.

    \If{$\left(\sum_{(\tau_r,\tau_c)\in{T}}{\|\wh{u}^{(\tau_r,\tau_c)}_j - a\omega^{-\tau_r i -\tau_c i'}\|} == 0 \right)$}
        \State $\wh{w}_{i,i'} \gets a$.
        \For{$(\tau_r,\tau_c)\in{T}$}
        \State $\wh{u}^{(\tau_r,\tau_c)}_j \gets 0$
        \If{IsCol}
        \State $\ell \gets i'\bmod B$
	\Else
	\State $\ell \gets i\bmod B$
        \EndIf
        \State $\wh{v}^{(\tau_r,\tau_c)}_{\ell} \gets \wh{v}^{(\tau_r,\tau_c)}_{\ell} -  a\omega^{-\tau_r i -\tau_c i' }$
        \EndFor
    \EndIf
    \EndFor
    \State \Return $\wh{w}$, $\wh{u}^{(T)}$, $\wh{v}^{(T)}$
    \EndProcedure
    \Procedure{Noiseless2DSparseFFT}{$x$, $k$}
    \State $B = \alpha k$, for some constant $\alpha$.
    \State $T \gets \{(0,0),(0,1),(1,0),(0,2),(2,0)\}$  \Comment{\textred{Verify that this is enough}}
    \For{$(\tau_r,\tau_c) \in T$}
    \State $\wh{u}^{(\tau_r,\tau_c)} \gets \textsc{FoldToBins}(x, B, 1, \tau_r, \tau_c)$.
    \State $\wh{v}^{(\tau_r,\tau_c)} \gets \textsc{FoldToBins}(x, 1, B, \tau_r, \tau_c)$.
    \EndFor
    \State $\wh{z} \gets 0$
    \For{$t \in 0,1, \dotsc, \log k$}
    \State $\{\wh{w}, \wh{u}^{(T)}, \wh{v}^{(T)}\} \gets \textsc{EstimateFreq}(\wh{u}^{(T)}, \wh{v}^{(T)}, T, B, $ true). \Comment{$\wh{u}^{(T)}=\{\wh{u}^{(\tau)}\,:\,\tau\in{T}\}$}
    \State $\wh{z} \gets \wh{z}  + \wh{w}$.
    \State $\{\wh{w}, \wh{v}^{(T)}, \wh{u}^{(T)}\}  \gets \textsc{EstimateFreq}(\wh{v}^{(T)}, \wh{u}^{(T)}, T, B, $ false).
    \State $\wh{z} \gets \wh{z}  + \wh{w}$.
    \EndFor
    \State \Return $\wh{z}$
    \EndProcedure
  \end{algorithmic}
\end{algorithm}



%\subsection{Exact Algorithm: $k = \Omega(\sqrt{n})$}



==> revision.tex <==
\newcommand{\Revision}{550}

